Implicit Distortion and Fertility Models for Attention-based Encoder-Decoder NMT Model

Neural machine translation has shown very promising results lately. Most NMT models follow the encoder-decoder framework. To make encoder-decoder models more flexible, attention mechanism was introduced to machine translation and also other tasks like speech recognition and image captioning. We observe that the quality of translation by attention-based encoder-decoder can be significantly damaged when the alignment is incorrect. We attribute these problems to the lack of distortion and fertility models. Aiming to resolve these problems, we propose new variations of attention-based encoder-decoder and compare them with other models on machine translation. Our proposed method achieved an improvement of 2 BLEU points over the original attention-based encoder-decoder.

==> sections/ram.tex <==
\subsection{RAM: Recurrent Models of Visual Attention}
\label{section:ram}
The visual recurrent attention model, RAM, uses a CNN as encoder and an RNN as decoder. The attention mechanism it uses follows:

$l_i=\text{Location}(h_{i-1})$
$c_i=\text{Glimpses}(l_i, \{s_j\})$
$h_i=\text{RNN}(h_{i-1}, c_i)$

where $\{s_j\}$ is the set of CNN output. This attention mechanism is purely location based. It first computes a location to focus on using a MLP (denoted as Location), then extracts information from that location using glimpse sensor (denoted as Glimpses). This is a hard attention \cite{xu2015show} where $l_t$ is chosen stochastically at each step.

